PupilNet v2.0: Convolutional Neural Networks for CPU based real time Robust Pupil Detection

Real-time, accurate, and robust pupil detection is an essential prerequisite for pervasive video-based eye-tracking. However, automated pupil detection in realworld scenarios has proven to be an intricate challenge due to fast illumination changes, pupil occlusion, non-centered and off-axis eye recording, as well as physiological eye characteristics. In this paper, we approach this challenge through: I) a convolutional neural network (CNN) running in real time on a single core, II) a novel computational intensive two stage CNN for accuracy improvement, and III) a fast propability distribution based refinement method as a practical alternative to II. We evaluate the proposed approaches against the state-of-the-art pupil detection algorithms, improving the detection rate up to ~9% percent points on average over all data sets (~7% on one CPU core 7ms). This evaluation was performed on over 135,000 images: 94,000 images from the literature, and 41,000 new hand-labeled and challenging images contributed by this work (v1.0).

==> tmpbib.tex <==
[2.] [683][690]
[4.] [170][186]
[5.] [317][335]
[6.] [1151][1160]
[11.] [163][170]
[14.] [78][87]
[15.] [2278][2324]
[16.] [3642][3649]
[17.] [1097][1105]
[18.] [9][48]
[20.] [381][395]
[24.] [77][80]
[29.] [392][407]
[30.] [354][370]
[31.] [1790][1798]
[32.] [3431][3440]
[33.] [3367][3375]
[34.] [82][90]
[35.] [2169][2178]
[36.] [54][115]
[38.] [195][204]
[39.] [75][80]
[40.] [199][233]

